Meta-learnt priors slow down catastrophic forgetting in neural networks

Current training regimes for deep learning usually involve exposure to a single task / dataset at a time. Here we start from the observation that in this context the trained model is not given any knowledge of anything outside its (single-task) training distribution, and has thus no way to learn parameters (i.e., feature detectors or policies) that could be helpful to solve other tasks, and to limit future interference with the acquired knowledge, and thus catastrophic forgetting. Here we show that catastrophic forgetting can be mitigated in a meta-learning context, by exposing a neural network to multiple tasks in a sequential manner during training. Finally, we present SeqFOMAML, a meta-learning algorithm that implements these principles, and we evaluate it on sequential learning problems composed by Omniglot and MiniImageNet classification tasks.

==> delete_all_auxs <==

previous formulation with L_i instead of F_tau



{\color{red}
The objective can formalized as
$$
    \minimize_{\boldsymbol{\phi}} \mathbb{E}_{T_1, T_2, \dots, T_n \sim p\left(T_{i\dots n}\right)} \left[ \frac{1}{n} \sum_{i=1}^n L_{i,\text{test}}\left(\boldsymbol{\tilde{\phi}}\right) \right]
$$
where $L_i(\boldsymbol{\phi})$ is the loss function of task $T_i$, $\boldsymbol{\tilde{\phi}}$ is the parameters vector obtained at the end of training on the sequence of tasks $T_1, \dots, T_n$, and $\boldsymbol{\tilde{\phi}}=\boldsymbol{\phi}^n=U_{n,\text{train}}^k( U_{n-1,\text{train}}^k( \dots U_{1,\text{train}}^k(\boldsymbol{\phi}) \dots ) )$. --Henceforth we will use the notation $\boldsymbol{\phi}^i$ to identify the parameters vector obtained after trainining on task $i$ and all the previous tasks, sequentially, $1, 2, \dots, i$.--

[Note that we can treat the full sequence of tasks as a single task whose behavior is non-stationary, and whole test function differs from its train function (e.g., for a sequence of classifiers, the training loss depends on the current dataset $i$ being used, but testing is performed on all the datasets combined).]
---
{\color{red}TODO}

$$
    \minimize_{\boldsymbol{\phi}} \mathbb{E}_{T_1, T_2, \dots, T_n \sim p\left(T_{i\dots n}\right)} \left[ \frac{1}{n} \sum_{i=1}^n L_{i,\text{test}}\left( \boldsymbol{\phi}^n \right) \right]
$$

SOLUTION 1: we follow the same approach as (FO)MAML, and compute the gradient of the meta-objective with respect to the initial parameters, and then optimize it by gradient descent
\begin{align*}
    g_\text{SeqMAML} &= \nabla_{\boldsymbol{\phi}} \mathbb{E}_{T_1, T_2, \dots, T_n \sim p\left(T_{i\dots n}\right)} \left[ \frac{1}{n} \sum_{i=1}^n L_{i,\text{test}}\left( \boldsymbol{\phi}^n \right) \right] \\
    &= \mathbb{E}_{T_1, T_2, \dots, T_n \sim p\left(T_{i\dots n}\right)} \left[ \frac{1}{n} \sum_{i=1}^n \nabla_{\boldsymbol{\phi}} L_{i,\text{test}}\left( \boldsymbol{\phi}^n \right) \right] \\
    &= \mathbb{E}_{T_1, T_2, \dots, T_n \sim p\left(T_{i\dots n}\right)} \left[ \frac{1}{n} \sum_{i=1}^n L_{i,\text{test}}'\left( \boldsymbol{\phi}^n \right) \frac{\partial \boldsymbol{\phi}^n}{\partial \boldsymbol{\phi}} \right] \\
    &= \mathbb{E}_{T_1, T_2, \dots, T_n \sim p\left(T_{i\dots n}\right)} \left[ \frac{1}{n} \frac{\partial \boldsymbol{\phi}^n}{\partial \boldsymbol{\phi}} \sum_{i=1}^n L_{i,\text{test}}'\left( \boldsymbol{\phi}^n \right) \right] \\
\end{align*}

where $\boldsymbol{\phi}^n$ are the final parameters obtained after training on the sampled sequence of tasks.
Note that the Jacobian term $\frac{\partial \boldsymbol{\phi}^n}{\partial \boldsymbol{\phi}}$ is the same for all the tasks in the sequence, as all tasks are evaluated at the same final parameters.
As in FOMAML, we can compute a first-order approximation of the meta-gradient by ignoring the second-order terms, replacing the Jacobian with the identity matrix
$$
    g_\text{SeqFOMAML} = \mathbb{E}_{T_1, T_2, \dots, T_n \sim p\left(T_{i\dots n}\right)} \left[ \frac{1}{n} \sum_{i=1}^n L_{i,\text{test}}'\left( \boldsymbol{\phi}^n \right) \right] \\
$$








\textbf{2) Then subsection on the sequential task loss / objectives / auxiliary gradients:
TODO: when I introduce the objectives: [also useful when i introduce the objectives: INSERT IN DISCUSSION: a sequence of task can be thought of a task itself, and this meta-learning would be the traditional one (as long as the loss of the task-as-sequence-of-tasks is given accordingly]}

{\color{red} IMPORTANT TO SAY:
all these losses work well, and the FO approx holds. However if the model is modified to add standard CL algos, the gradients may change and this may not hold anymore. Ideally, we'd use derivatives-free optimization.  For some models, it should be possible to derive the functionals anyway {\color{red} FOR ICML, MUST INCLUDE SI and Hebbian!}}





Problem: the final test curves (avg performance on previously seen tasks after training on each task in a sequence) starts very low and grows fast within the seq-length used during training. This is because the objective we use really is encouraging positive backward transfer, as the initial performance of tasks doesn't matter -- only their performance at the end of the full sequence is optimized. We can try and address it in two related ways:

\subsubsection{Method 1}

More accurate, but computationally more expensive. And also, not task agnostic (during meta-training, but after it is)  After training on each task, compute the gradient of loss of the current task at the current parameters, with respect to the initial parameters
$$
    g_{\text{aux}} = \frac{\partial L_{i,\text{test}}(\boldsymbol{\phi}^i)}{\partial \boldsymbol{\phi}} = U_{i,\text{train}}^{i'}(\boldsymbol{\phi}) L_{i,\text{test}}'(\boldsymbol{\phi}^i) \approx L_{i,\text{test}}'(\boldsymbol{\phi}^i)
$$
where we use the notation $\boldsymbol{\phi}^i$ to mark the parameters vector of the model after finishing training on task $i$ within the sequence.

So the final gradient becomes
$$
    g_\text{SeqFOMAML} + g_{\text{aux}} = \mathbb{E}_{T_1, T_2, \dots, T_n \sim p\left(T_{i\dots n}\right)} \left[ \frac{1}{n} \sum_{i=1}^n L_{i,\text{test}}'\left( \boldsymbol{\phi}^n \right) + L_{i,\text{test}}'(\boldsymbol{\phi}^i) \right] \\
$$

--- note: perf at phi i enforces learning quickly (i.e., the final performance is not only due to backward transfer!); perf at phi n enforces backward transfer and reducing catastrophic forgetting

\subsubsection{Method 2 - enforce performance during training}

Another way is to explicitly minimize the test loss of each task in the sequence after training on each other task. Namely
$$
    \minimize \mathbb{E}_{T_1, T_2, \dots, T_n \sim p\left(T_{i\dots n}\right)} \left[ \frac{1}{n} \sum_{i=1}^n \sum_{j \leq i} \frac{L_{j,\text{test}}(\boldsymbol{\phi}^i)}{n+1-j} \right]
$$

Note that the loop iteration for $j=i$ is the same as the original SeqFOMAML objective. We divide each loss by $n+1-j$ so that each task presented in the sequence contributes equally to the objective.

Finally, we test an approximation in which a single previous task (or a fixed number $m<n$) is sampled after training on each task, to keep the computational complexity of the loss linear in the length of the sequence, rather than quadratic
$$
    \minimize \mathbb{E}_{T_1, T_2, \dots, T_n \sim p\left(T_{i\dots n}\right)} \left[ \frac{1}{n} \sum_{i=1}^n L_{j,\text{test}}(\boldsymbol{\phi}^n) + L_{j \sim U([0,i]),\text{test}}(\boldsymbol{\phi}^i) \right]
$$

}








